Analytic Provenance Datasets: A Data Repository of Human Analysis Activity and Interaction Logs

We present an analytic provenance data repository that can be used to study human analysis activity, thought processes, and software interaction with visual analysis tools during exploratory data analysis. We conducted a series of user studies involving exploratory data analysis scenario with textual and cyber security data. Interactions logs, think-alouds, videos and all coded data in this study are available online for research purposes. Analysis sessions are segmented in multiple sub-task steps based on user think-alouds, video and audios captured during the studies. These analytic provenance datasets can be used for research involving tools and techniques for analyzing interaction logs and analysis history. By providing high-quality coded data along with interaction logs, it is possible to compare algorithmic data processing techniques to the ground-truth records of analysis history.

==> files/2-userInteraction.tex <==

% \begin{center}
% \begin{figure*}[!t]
%  \centering 
%  \includegraphics[width=6.8in]{figures/2-3.png}
% %  \includegraphics[width=6.8in]{figures/cyber_data.png}
%  \caption{Screenshot of the document analysis tool used for collecting provenance data in the user studies.
%  All text documents are listed in a collapsed format with a random order on the left monitor at the beginning of the study.
%  Documents have titles and users are able to drag and displace documents in the explorer tool space.
%  In this tool user can write notes, move and link documents, highlight text and search words.
%  }
%  \label{fig:Exptool}
% \end{figure*}
% \end{center} 

% \begin{table}[!b]
%   \centering
%   \begin{tabular}{r l}
%      \toprule
%     %& \multicolumn{2}{c}{\small{\textbf{Meaning}}} \\
%     \cmidrule(r){1-2}
%     {\small\textbf{Interactions}}
%     & {\small \textbf{Purpose}} \\
%     %& {\small \textit{Translation}} \\
%     \midrule
%     Open documents & Explore new articles \\% & Looking for new articles \\
%     Read documents & Explore new information \\% & Reading an open article \\
%     Search & Keyword search \\ %& Searching a key word or date \\
%     Highlight & Highlight document text \\%& Highlighting article contexts \\
%     Bookmark & Select documents \\
%     Connect & Linking documents and notes\\%\\& Make connection between articles \\
%     Move documents & Arrange documents in screen \\%& Displace articles in the screen \\
%     Brush titles & Review document titles \\
%     Creating Notes & Making sticky notes \\%& Making notes \\    
%     Writing Notes & Writing notes %& Making notes \\    

%     % \bottomrule
%   \end{tabular}
%   \caption{Types of interactions logged from the text analysis tool during the user studies.
%   }~\label{tab:table1}
% \end{table}


% \subsection{Text Analysis Dataset}

% To complete the analysis task, participants used a basic visual analysis tool (see Figure~\ref{fig:Exptool} on next page.
% The tool supports spatial arrangement of articles, the ability to link documents, keyword searching, highlighting, and note-taking.
% When loading the data in our document explorer tool, each document starts as collapsed with only its title visible.
% Users could ``open'' any document by double-clicking the title bar or by clicking a dedicated button on the document's title bar, and this would expand the document to a window containing the text of the document.
% The document could be collapsed back to the title in the same way.
% Within an open document, users could highlight text by selecting it, right-clicking, and activating a menu item.
% When a window has highlighted text, the window could be ``reduced to highlight'', which would hide all text in the document except for the highlighted content.
% At the beginning of the study, documents were arranged in the left screen without a specific order or grouping.
% Users clicked and dragged documents, freely re-arranging documents in the workspace.
% They could also create editable notes windows in the same workspace.
% When using the \textit{search} functionality, both matching words within windows and the windows themselves were highlighted.
% Users could also draw connection lines across document windows, which created a line to denote relationships visually.

% All user interactions at a rudimentary level like mouse movements and clicks are captured during the study using the text explorer.
% Later we transform basic data log recorded from explorer tool to nine type of user actions, see Table ~\ref{tab:table1}.
% We associate analytical reasoning with different interactions available to the user, and later use it to modify the topic models.

% Based on prior observations (e.g.,~\cite{MouseRef,goecks2000learning})  that mouse input can correspond with informational attentional. 
% We use hovering the mouse over new document titles as users intend to explore new information.
% Hovering mouse over document text shows reading interaction of the articles.


% \subsection{Cyber Analysis Dataset}

% Participants are given the task to explore the multidimensional dataset to determine the suspicious behavior.
% A static view of the tool is shown in Figure ~\ref{fig:Cybertool}.
% The tool is divided into following 6 different views described in~\ref{tab:cybertable}
% % The tool is divided into following 6 different views:
% % \begin{itemize}\compresslist%
% % \item Overview histogram of monthly network traffic with a time bin of 1 day.
% % \item Detailed histogram of the traffic shown with smaller time bin.
% % \item Connected network graphs between different IP addresses. 
% % \item Office view with workspace IP shown with employee ID.
% % \item Information box for familiarization of the tool.
% % \item IP tables with detailed network traffic data.
% % \end{itemize}
% % \begin{table}[!t]
% %   \centering
% %   \begin{tabular}{l}
% %      \toprule
% %     \cmidrule(r){1-1}
% %     {\small\textbf{Cyber analysis tool's views}} \\
% %     \midrule
% %     Overview histogram of monthly network traffic \\
% %     Detailed histogram of hourly network traffic\\
% %     Network graphs between different IP addresses \\ 
% %     Office view with workspace IP and the employee ID \\
% %     Information box for familiarization of the tool \\
% %     IP tables with detailed network traffic data
% %     % \bottomrule
% %   \end{tabular}
% %   \caption{Types of eye and mouse interactions logged from the cyber analysis tool during the user studies.
% %   }~\label{tab:cybertable}
% % \end{table}
% % \begin{table*}[!t]
% %   \centering
% %   \begin{tabular}{l l l}
% %      \toprule
% %     \cmidrule(r){1-3}
% %     {\small\textbf{Eye Area of Interest (AOI)}}
% %     & {\small \textbf{Mouse interaction Data logs}}
% %     & {\small \textbf{Mouse interaction Data logs}} \\
% %     \midrule
% %     Overview Histogram & Brush Start and End & Overview histogram of monthly network traffic \\
% %     Detailed Histogram & Mouse Enter and Bar Click & Detailed histogram of hourly network traffic\\
% %     Network Graph & Mouse Enter & Network graphs between different IP addresses \\ 
% %     Office View & Mouse Enter, Click and Slider move & Office view with workspace IP and the employee ID \\
% %     Information Box & Mouse Hover & Information box for familiarization of the tool \\
% %     IP Table & Click, Page Change and Row Select & IP tables with detailed network traffic data
% %     % \bottomrule
% %   \end{tabular}
% %   \caption{Types of eye and mouse interactions logged from the cyber analysis tool during the user studies.
% %   }~\label{tab:cybertable}
% % \end{table*}
% \begin{table}[!b]
%   \centering
%   \begin{tabular}{r l}
%      \toprule
%     %& \multicolumn{2}{c}{\small{\textbf{Meaning}}} \\
%     \cmidrule(r){1-2}
%     {\small\textbf{Eye Area of Interest (AOI)}}
%     & {\small \textbf{Mouse interaction Data logs}} \\
%     %& {\small \textit{Translation}} \\
%     \midrule
%     Overview histogram & Brush start and end \\
%     Detailed histogram & Mouse enter and bar click \\
%     Network graph & Mouse enter \\ 
%     Office view & Mouse click and slider move\\
%     Information box & Mouse hover \\
%     IP table & Page change and row select \\
%     % \bottomrule
%   \end{tabular}
%   \caption{Types of eye and mouse interactions logged from the cyber analysis tool during the user studies.
%   }~\label{tab:cybertable}
% \end{table}
% Due to huge amount of data, filtering is required to find specific patterns in the data.
% Brushing and linking is enabled in the overview histogram view.
% Any portion of it can be selected and then the detailed histogram will change according to the selection.
% Office view shows the current status of the employees inside embassy in that specific time frame using different color codes.
% A slider tool also allows the participant to select specific time and day to check the employee status and network traffic.
% Moreover, participants can select specific IP addresses from a multi-paged IP table for future reference.
% User interactions with the tool is recorded in the form of mouse interaction and eye area of interest (AOI). 
% % Mouse tracking is done within the tool and it is consist of mouse hover and click events, slider move events, table pages and row selections. 
% Mouse tracking is done within the tool while eye tracking is performed using a Tobii EyeX, a standard eye tracking device that tracks the eye gaze fixation points. 


% \begin{center}
% \begin{figure}[!t]
%  \centering 
%  \includegraphics[width=1.0\columnwidth]{figures/cyber_data.png}
% %  \includegraphics[width=6.8in]{figures/cyber_data.png}
%  \caption{Screenshot of the cyber analysis tool used for collecting provenance data in the user studies. 
%  Charts on the top left sides are detailed histogram and overview histogram, respectively. 
%  A network graph is shown in the bottom left. 
%  Boxes on the top right corner indicates the office view with slider tools.
%  Below the office view is an information panel.
%  Finally, at the bottom right, an IP traffic table shows detailed network data.  }
%  \label{fig:Cybertool}
% \end{figure}
% \end{center} 


% \begin{center}
% \begin{figure*}[!t]
%  \centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
%  \includegraphics[width=\textwidth,height=6cm]{figures/cyber_data.png}
%  \caption{Screenshot of the cyber data analysis tool
%  }
%  \label{fig:Cybertool}
% \end{figure*}
% \end{center} 
